The Hadronic Final State at HERA

The hadronic final state in electron-proton collisions at HERA has provided a rich testing ground for development of the theory of the strong force, QCD. In this review, over 200 publications from the H1 and ZEUS Collaborations are summarised. Short distance physics, the measurement of processes at high energy scales, has provided rigorous tests of perturbative QCD and constrained the structure of the proton as well as allowing precise measurements of the strong coupling constant to be made. Non-perturbative or low energy processes have also been investigated and results on hadronisation interpreted together with those from other experiments. Searches for exotic QCD objects, such as pentaquarks, glueballs and instantons have been performed. The subject of diffraction has been re-invigorated through its precise measurement, such that it can now be described by perturbative QCD. After discussion of HERA, the H1 and ZEUS detectors and the techniques used to reconstruct differing hadronic final states, the above subject areas are elaborated. The major achievements are then condensed further in a final section summarising what has been learned.

==> searches.tex <==
\section{Searches in the Final State}

\begin{itemize}
   \item {\bf Estimated length:} 7 pages
\end{itemize}

\subsection{Exotic and Unusual QCD} 
\label{sec:exo-qcd}

The main focus 
of this short section is to take a fresh look at pentaquark data 
after the dust has settled. Unless the final HERA-II data confirm the HERA-I
evidence, this will mainly just be to note the conclusion that
these studies ultimately did not come to much.  

Pentaquarks papers~\cite{Aktas:2004qf,Aktas:2006ic,Aktas:2007dd,Chekanov:2004kn,Chekanov:2004qm,Chekanov:2005at} of which : 
$\Xi\pi$~\cite{Chekanov:2005at,Aktas:2007dd}; $D^*p$~\cite{Aktas:2004qf,Chekanov:2004qm,Krueger:2009zz}; and 
$K_S^0 p$~\cite{Chekanov:2004kn,Aktas:2006ic} ...

Odderons~\cite{Adloff:2002dw} ...

Instantons~\cite{Adloff:2002ph,Chekanov:2003ww} ...

Glueballs~\cite{Chekanov:2003wc,Chekanov:2008ad}, see Fig.~\ref{fig:ks-ks} ...

\begin{figure}[htp]
\begin{center}
~\epsfig{file=Figures/Searches/DESY-08-068_2.eps,height=8cm}
\caption{(a) The measured $K_S^0 K_S^0$ invariant-mass spectrum compared to a fit of signal and background.  (b) The 
background-subtracted $K_S^0 K_S^0$ invariant-mass spectrum with the fit for the signals also shown.  
From~\cite{Chekanov:2008ad}.}
\label{fig:ks-ks}
\end{center}
\end{figure}

Deuterons~\cite{Aktas:2004pq,Chekanov:2007mv} ...

\begin{figure}[htp]
\begin{center}
\vspace{1cm}
~\epsfig{file=Figures/Searches/DESY-07-070_9.eps,height=7cm}
\caption{From~\cite{Chekanov:2007mv}}
\label{fig:deuteron}
\end{center}
\end{figure}


\subsection{Searches for BSM Physics}

Here, we plan to adopt an approach based around experimental signatures. 
This may bring 
something complementary to the presumably more model based 
review \cite{nachtman:grivaz} (which we will of course rely on via
citations for many missing topics, SUSY channels in particular).
We will also refer to \cite{max:mandy} for limits 
from inclusive measurements, such as contact interactions.

The section could begin by reviewing the `General' search papers, in which 
any multiplicity and combination of high transverse momentum $e$, $\mu$, 
$\gamma$, jet and $\nu$ is studied and compared with models, concluding 
that the data in extreme high pt corners of phase space 
are well understood and nothing really striking sticks out. The possible
exception is the H1 `isolated lepton' signal involving a
high $p_T$ lepton, missing $E_T$ and a large hadronic $p_T$ 
(dominated by $W$ production in the standard model). 

The final significance of the isolated lepton signal will be discussed 
(likely about $3 \sigma$ in H1 with nothing anomalous seen in ZEUS). No
strong conclusions will be drawn at that level of significance, though
the results of attempts to interpret it in terms of single top production
via a flavour changing neutral current and $\tilde{t}$ production will
be mentioned. 

In similar style, we also anticipate a brief discussion of the 
lack of any exotic signal in the channels to which HERA is most sensitive:
lepton+jet resonances (leptoquarks,squarks) and excited electrons, neutrinos 
and quarks decaying to lepton + photon.

\begin{itemize}
   \item {\bf Probable Figure:} Summary figure of multi-topology `general
search'
   \item {\bf Probable Figure:} `Isolated lepton' signals from H1 and ZEUS
   \item {\bf Probable Figure:} Limit plot for leptoquarks    
   \item {\bf Probable Figure:} Example limit plot for excited fermions
\end{itemize}



